Optimized Kernel-based Projection Space of Riemannian Manifolds

It is proven that encoding images and videos through Symmetric Positive Definite (SPD) matrices, and considering the Riemannian geometry of the resulting space, can lead to increased classification performance. Taking into account manifold geometry is typically done via embedding the manifolds in tangent spaces, or Reproducing Kernel Hilbert Spaces (RKHS). Recently, it was shown that embedding such manifolds into a Random Projection Spaces (RPS), rather than RKHS or tangent space, leads to higher classification and clustering performance. However, based on structure and dimensionality of the randomly generated hyperplanes, the classification performance over RPS may vary significantly. In addition, fine-tuning RPS is data expensive (as it requires validation-data), time consuming, and resource demanding. In this paper, we introduce an approach to learn an optimized kernel-based projection (with fixed dimensionality), by employing the concept of subspace clustering. As such, we encode the association of data points to the underlying subspace of each point, to generate meaningful hyperplanes. Further, we adopt the concept of dictionary learning and sparse coding, and discriminative analysis, for the optimized kernel-based projection space (OPS) on SPD manifolds. We validate our algorithm on several classification tasks. The experiment results also demonstrate that the proposed method outperforms state-of-the-art methods on such manifolds.

==> temp.tex <==
We build the local similarity graph by solving use local information
around each point to build a similarity between pairs of
points. These methods are known to have limitations when it comes to dealing with
points near the intersection of two subspaces

resolve these issues by building better similarities between
data points using global information.

The solution of the
corresponding global optimization algorithm is then used
to build a similarity graph from which the segmentation of the data is obtained.


local and global similarity graphs
each data point, we find a few other points that belong to
the same subspace. To do so, we propose to employ local and global sparse optimization program whose solution encodes information
about the memberships of data points to the underlying
subspace of each point.
Weighted graph 
A method consists of both local and global spectrul clustering, Local spectral clustering methods, use local information
around each point to build a similarity between pairs of
points.
These methods have difficulties in dealing with
points near the intersection of two subspaces because the
neighborhood of a point can contain points from different
subspaces. In addition, they are sensitive to the right choice
of the neighborhood size to compute the local information
at each point.
Global spectral clustering-based approaches try to
resolve these issues by building better similarities between
data points using global information

The solution of the
corresponding global optimization algorithm is then used
to build a similarity graph from which the segmentation of
2766 IEEE TRANSACTIONS ON PATTERN ANALYSIS AND MACHINE INTELLIGENCE, VOL. 35, NO. 11, NOVEMBER 2013
Fig. 2. Face clustering: Given face images of multiple subjects (top), the goal is to find images that belong to the same subject (bottom).
Fig. 1. Motion segmentation: Given feature points on multiple rigidly moving objects tracked in multiple frames of a video (top), the goal is to separate
the feature trajectories according to the moving objects (bottom).
the data is obtained.
